Checks and Balances: A Low-complexity High-gain Uplink Power Controller for CoMP

Coordinated Multipoint (CoMP) promised substantial throughput gain for next-generation cellular systems. However, realizing this gain is costly in terms of pilots and backhaul bandwidth, and may require substantial modifications in physicallayer hardware. Targeting efficient throughput gain, we develop a novel coordinated power control scheme for uplink cellular networks called Checks and Balances (C&B), which checks the received signal strength of one user and its generated interference to neighboring base stations, and balances the two. C&B has some highly attractive advantages: C&B (i) can be implemented easily in software, (ii) does not require to upgrade non-CoMP physicallayer hardware, (iii) allows for fully distributed implementation for each user equipment (UE), and (iv) does not need extra pilots or backhaul communications. We evaluate the throughput performance of C&B on an uplink LTE system-level simulation platform, which is carefully calibrated with Huawei. Our simulation results show that C&B achieves much better throughput performance, compared to several widely-used power control schemes.

==> GlobeCom16_Sumbmission/Abstract.tex <==
\begin{abstract}
%In this paper, we focus on practical CoMP technique design from the point of view in open-loop uplink power control problem. A novel coordinated open-loop power control solution named \emph{Checks and Balances (C\&B)} is proposed, which only exploit large-scale path losses and system priori knowledge. Testified via system-level simulations, C\&B provides significant performance improvements in terms of cell average throughput, cell-edge throughput and power saving, over existing non-coordinated and coordinated open-loop power control approaches. Furthermore, C\&B's complexity and implementation requirement remain low, thereby can be easily adopted in practical uses.
%Coordinated Multipoint is the term used to refer to base station coordination in cellular networks. There has been numerous proposals in the literature, showing substantial gains over non-coordinated solutions under idealized conditions. However, no significant approach has been adopted in practice, since the tight constraints on practical factors such as backhaul latency, computational complexity, and channel estimation render most of these solutions unfeasible in current LTE systems. To that end, we propose an uplink open-loop power control scheme, Checks and Balances, which exploits large-scale channel variations to choose transmission power levels of mobile units, cooperatively across neighboring cells. Using a carefully-calibrated system-level LTE simulator, we respectively show a $51.9\%$ improvement on the average cell throughput and a $156\%$ improvement on the edge-user throughput over two widely adopted non-coordinated industry standard power control schemes. Further, our scheme outperforms a recently proposed candidate coordinated power control approach by providing a $25.1\%$ gain in average cell throughput. Checks and Balances is carefully designed to meet the LTE system-design constraints specified by 3GPP standards and it incurs only a minimal additional cost on coordination and complexity over the existing non-coordinated solutions.
Coordinated Multipoint (CoMP) techniques have promised substantial throughput improvement by exploiting the cooperation across base stations in cellular networks. In addition to the high computation and implementation complexity, existing CoMP proposals also require different base stations to exchange co-channel condition information through backhaul links. Such cooperation incurs additional costs in pilots and backhaul bandwidth, which in turn reduces the resource allocated to data transmission. Therefore, the promised throughput gain is greatly degraded in practical applications. Aiming to overcome this limitation, we develop a novel coordinated power control scheme for uplink cellular networks, named Checks and Balances (C\&B) , which can realize the potential benefits of CoMP with minimum complexity and cost. C\&B checks the signal strength of one user and its generated interference to neighboring base stations, and tries to balance the two. We evaluate the throughput performance of C\&B on an LTE system-level simulation platform, which is carefully calibrated with Huawei. Our simulation results suggest that C\&B achieves up to $52\%$ increase in average throughput, and up to $156\%$ increase in edge-user throughput, compared to existing power control schemes.
%C\&B is shown to provide a $51.9\%$ improvement on the average throughput per cell over the widely adopted Fractional Power Control (FPC) scheme. In additional comparison with Max Power policy, C\&B improves the edge-user throughput and power efficiency by $156\%$ and $5,716\%$, respectively.    
\end{abstract}
\begin{IEEEkeywords}
Uplink power control, coordinated multipoint (CoMP), LTE, system-level simulation, throughput improvement
\end{IEEEkeywords}

==> GlobeCom16_Sumbmission/Conclusion.tex <==
\section{Conclusion and Future Work}\label{Conclusion}
%We studied the power control problem for uplink cellular networks. Even though, it is not
%possible to achieve the optimal solution due to the strong NP hardness, we
%proposed a novel power control scheme named \emph{Checks and Balances (C\&B)}, that has low complexity, low implementation requirements and high universality to various circumstance. Verified by system-level simulations, C\&B respectively achieves a $51.9\%$ improvement on the average cell throughput and a $156\%$ improvement on the edge-user throughput over two widely adopted non-coordinated industry standard power control schemes. Further, C\&B outperforms a recently proposed candidate CoMP power control scheme by providing a $25.1\%$ cell average throughput improvement. Note that all the performance gains are obtained solely by our proposed coordinated open-loop power control scheme. Implementing other CoMP techniques such as CoMP scheduling and closed-loop power control in combination with C\&B may further improve the throughput performance, which are the future directions of our research. 
We investigate how to use limited large scale CSI to achieve the throughput gain of CoMP through the design of a power controller named C\&B. The optimal power control by itself is an NP hard problem, which has been open up to date. Further, as very limited coordination is possible in the open-loop mode, the power controllers of different BSs are not allowed to communicate. C\&B satisfies all practical constraints in cellular systems, and can significantly improve the average and edge throughput over existing power control schemes with very low complexity and almost no cost. Further throughput enhancement is promising by combining C\&B with other coordinated transceiver and scheduling techniques.

==> GlobeCom16_Sumbmission/Intro.tex <==
\section{Introduction}
Next generation of cellular communication, e.g., Long Term Evolution Advanced (LTE-A) and 5G, is expected to significantly improve the average throughput and cell-edge throughput for serving user equipments (UEs).
% In cellular networks, 
%base stations (BS) are further divided into different cells\footnote{In this paper, we regard one sector of a BS as one cell.}. 
%enormous non-coordinated transmitters and receivers are using the same spectrum that makes the system interference-limited. 
One important candidate technique for achieving such throughput improvement is Coordinated Multipoint (CoMP), which refers to the cooperation among different Base Stations (BSs).
%One of the directions for potential improvement is the cooperation among different cells\footnote{In this paper, we regard each sector of a BS as one cell.} of a Base Station (BS) as well as different BSs, i.e. Coordinated Multipoint (CoMP). 

It has been observed that  the benefits of CoMP are hard to be realized due to many practical issues \cite{Lozano13, Suh11}, which may even lead to a lower throughput than non-CoMP techniques \cite{Barbieri12}. In particular, the uplink CoMP techniques such as cooperative interference cancellation/alignment, beamforming, and scheduling all require different BSs to exchange scheduling, beamforming and channel state information through backhaul links. Acquiring such information incurs excessive costs in pilots and backhaul bandwidth, which results in considerable decrease in the resource allocated for data transmission. Further, the additional latency caused by backhaul communication \cite{36.213} makes the exchanged channel station information (CSI) outdated. Therefore, the expected throughput gain is greatly degraded. 

%The key practical limitations include: (1) feedback cost, e.g. the data rate consumed in feedback transmission; (2) Limited capability of backhaul links, e.g. latency and throughput constraint; (3) 
 %One of the directions for potential improvement is Coordinated Multipoint (CoMP), which is the term used to describe methods and techniques that utilize coordination among different cells of a Base Station (BS) as well as different BSs.  

%In this paper, we propose an open-loop power control scheme that provides substantial throughput gains over the existing industry standard Fractional Power Control (FPC) and Max Power schemes, without an increase in latency\footnote{Latency can be due to (1) required signaling for the algorithm (e.g., closed-loop) to converge, (2) estimation (e.g., additional pilots, etc.), (3) high computational complexity,(4) extra overhead processing.} and at a minimal increase in computational complexity. In a typical macrocell setting, we demonstrated an average throughput improvement of $54.2\%$ at almost the same edge-throughput as FPC, and an edge-throughput improvement of $144\%$ at approximately the same average throughput as Max Power scheme. Furthermore, the proposed scheme provides a controlled amount of improvement on edge vs. average throughput, depending on the choice of its parameter.

%Therefore, a critical question is ``is CoMP technique just a beauty of myth that out of the reach for realistic uses?'' We aim to answer this question by studying the open-loop power control problem in uplink cellular networks and proposing a practical solution with significant throughput improvement.

%In wireless propagation, path loss is separated into two components, large-scale and small-scale. Large-scale is due to longer-term effects caused by factors such as shadowing, distance-dependent path loss, penetration loss and antenna pattern, while small-scale is due to scattering combined with mobility, leading to fast fading. Thus, here `scale' refers to the time scale. In uplink cellular networks, open-loop power control refers to a MAC layer technique that sets the transmission power of one UE, by exploiting its large-scale path losses. The crucial requirements include low complexity, low and simple control signaling exchange, low-delay in backhaul links, eliminating those based on feedback/iterative adjustments. While coordination has substantial potential gains, the constraints imposed by the aforementioned requirements eliminated the adoption of existing physical-layer CoMP techniques. Indeed, \cite{Novlan13}-\cite{Castellanos08} show that the gains associated with existing solutions remain low and \cite{Xiao06} experienced a loss in the overall performance with all constraints taken into account. A thorough study of limitations of coordination can be found in \cite{Lozano13}.
%[cite some papers about cooperation gain in theory, e.g. DIDO etc.]

%Hence, open-loop power control eliminate the negative impacts of inevitable constraints in realistic cellular systems, e.g. system delay, backhaul, overheads cost, sophisticated signal processing. Note that these constraints prevent advanced physical layer CoMP techniques from being adopted in practice \cite{Lozano13,Suh11,Barbieri12}. By properly allocating transmission power to the scheduled UEs, the throughput performance can be significantly improved and robust to network dynamics.
Aiming to realize the potential benefits of CoMP in practical systems, we propose a novel coordinated power control design for uplink cellular networks. The task of uplink power control is to make the signal received  at the base station sufficiently strong, and in the meanwhile keep the interference generated to nearby base stations not severe. In practice, overly high and overly low transmission powers are both harmful. Specifically, increasing the transmission power of one UE can increase its  throughput, but it causes some strong interference to nearby cells, which will degrade the throughput of other UEs. Hence, finding the correct balance between a UE's own performance and its incurred cost to the other UEs is crucial to achieve a satisfying performance.

In practical uplink cellular networks, one UE's signal experiences the interference from hundreds of UEs from neighboring cells. Even if perfect CSI knowledge of the signal and interference channels are available, the optimal power control problem is strongly NP hard \cite{Shah11,Luo08}. To make things worse, the base station in current systems typically estimates the signal channel of its served UEs, but the channels of interfering UEs are mostly unavailable for estimation. These practical limitations makes the power control problem even more challenging.

%The base station in current systems typically estimates the individual channel of its served UE, but the channels of interfering UEs are unavailable in most part. Further, even with perfect CSI knowledge for all channels, the optimal power control by itself is proved to be strongly NP hard \cite{Shah11,Luo08}. Under such practical limitations, power control problem becomes extremely challenging.
%Designing desirable power control scheme is not easy. The optimal power control by itself is proved to be strongly NP hard even with perfect CSI \cite{Shah11,Luo08}. Further, when CSI is imperfect, this problem is even more difficult. In real systems, there are a huge population of users with diverse channel conditions, and channel knowledge is only available for a small amount of local wireless links. Any extra CSI exchange across different BSs results in additional costs in pilots and backhaul bandwidth. 
%The uplink power control cannot be reduced to a single cell problem because the UEs that served in one cell simultaneously interfere their neighboring cells. Unfortunately, the joint power allocation optimization for all UEs across all BSs is proved to be strongly NP hard even with perfect CSI \cite{Shah11,Luo08}. Further, when CSI is imperfect, this problem is even more difficult.  In spite of these notorious difficulties, the aforementioned practical limitations make the cooperative optimization across only a few BSs not feasible in practice.

%One of the main challenges in power control is that, the cellular network is interference-limited, and it was proven in \cite{Shah11,Luo08} that optimal power control is \emph{strongly NP hard} for co-interference channel even with perfect channel state information (CSI). Further, when CSI is imperfect, this problem is even more difficult. Consequently, the field of power control in cellular networks has been mainly dedicated to the development of suboptimal solutions that achieve a high performance. Some such approaches include the following.

%Contemporary cellular networks, e.g. 3G and LTE, handle the power allocation problem by constructing a slow mode power control which is only executed once in every tens of milliseconds (e.g. 50 ms) \cite{36.213}, i.e. open-loop power control. Under such control, the transmission power of each UE is allocated based on the accumulated time-average CSI, which is also referred to large-scale path loss. This significantly reduce the requirements on the amount and accuracy of CSI, but the throughput performance of existing solutions is unsatisfying. To this end, we are motivated to improve the open-loop power control design.


%CDMA-based systems (e.g. 3G networks) widely adopt Full Compensation Power Control (FCPC), aiming to alleviate the near-far problem\footnote{All UEs within a cell are transmitting  on the same spectrum in CDMA-based systems. The nearby UE has to carefully select its transmission power in order not to overwhelm the signals sent from faraway UEs in the same cell.} caused by strong intra-cell interference. FCPC allocates transmission power to one UE by making full compensation of its large-scale path loss such that all UEs have the same received signal strength, which results in poor performance in per-cell average throughput and inter-cell interference management.

%By employing single-carrier frequency division multiple access (SC-FDMA) techniques, 4G networks (e.g. LTE) assign UEs within one cell with orthogonal spectrums. This eliminates intra-cell interference in most part, but the problem of inter-cell interference remains. FPC allocates transmission power by making fractional compensation of UEs' large-scale path losses, such that UEs in the interior of one cell have stronger received signal strength than UEs at the cell edge. FPC performs much better than FCPC in reducing inter-cell interference, but the cell average throughput remains unsatisfactory. As an alternative power control scheme which focuses on cell average throughput improvement, Max Power allocates all UEs with the maximum allowable transmission power. Though the cell average throughput is greatly increased, Max Power performs a lot worse than FPC in terms of power efficiency and throughput of UEs at the cell edge \cite{Furuskar08, Castellanos08}. Hence, FPC is currently the most widely adopted non-coordinated open-loop power control scheme. Calibration of FPC to enhance the network performance draws a lot research interests from both theoretical and practical point of views \cite{Andrews13, Novlan13, Xiao06, Coupechoux11}.

%Furthermore, Full Compensation Power Control has an unsatisfactory average throughput due to high inter-cell interference.
%While in LTE cellular networks, SC-FDMA air interfaces are implemented. It makes intra-cell interference negligible and thereby no longer the biggest concern. Therefore, the key idea of this scheme is not applicable in LTE networks. Its main drawbacks come from cell average throughput and inter-cell interference management performance. 
%In Max Power scheme, all UEs transmit at their maximum allowable power. Compared with Full Compensation Power Control, it provides better average throughput per cell. However, the performance of cell-edge UE throughput, power efficiency and interference management become much worse. FPC set the transmission power of a UE by fractionally compensate its large scale path loss estimate \cite{Whitehead}. It is testified to have preferable advantages over both Full Compensation and Max Power schemes, providing noticeable performance improvement on their individual shortcomings \cite{Furuskar08, Castellanos08}. Hence, FPC is currently the most widely adopted Non-CoMP open-loop power control scheme. Calibration of FPC to enhance the network performance draws a lot research interests from both theoretical and practical point of views \cite{Andrews13, Novlan13, Xiao06, Coupechoux11}.

 
% It is essentially a modified version of FPC, which takes extra fractional compensation for the large-scale path loss of one UE's strongest interference link\footnote{We refer interference links to those between a UE and its nearby cells. And the link connecting a UE with its serving cell is referred to signal link.}. 
%Compared with FPC, it increases the cell average throughput by $20\%$. A similar scheme is also proposed in \cite{Yang09}. However, these two schemes are essentially group-wise FCPC: they put UEs into different groups based on the difference of large-scale path losses from one UE to its serving cell and neighboring cells, and intend to let them achieve group-specific received signal strength. Hence, they partially inherit the drawbacks of FCPC which significantly limits the throughput gain.  

%These two schemes put UEs into different groups based on the difference of large-scale path losses from one UE to its serving cell and neighboring cells, and set the transmission power such that all UEs within one group achieve the same large-scale signal strength. However, the absolute values of path losses are omitted. This leads to the same drawback of Full Compensation Power Control, which limits the potential throughput improvement of coordinated power control. 
%The findings indicate the advantage of coordinated power control, which worths further investigation.


%The objective of open-loop power control is to guarantee strong enough received signal and keep low enough co-channel interference. Existing non-coordinated power control approaches, as standardized in \cite{36.213}, make various levels of compensation for the large-scale path losses from UEs to their serving cells. To complement the lack of explicit consideration for co-channel interference, existing coordinated power control approaches \cite{Rao07}-\cite{Yang09} take additional compensations of large-scale path losses from UEs to their neighboring cells. 
%The strongly NP hardness of optimal solution, practical issues and unsatisfactory performance of existing approaches make the uplink power control an open problem for several decades, which motivates us to seek new practical scheme design. 
In our research, we develop a low-complexity CoMP-based power control scheme that provides significant throughput gains over the non-CoMP options, while using minimal additional resources for information exchange among base stations. To that end, the following are the contributions of this paper:
\begin{itemize}
\item We develop a novel coordinated power control scheme, named Checks and Balances (C\&B). %which can realize the potential benefits of CoMP with minimum complexity and cost. 
C\&B requires very little information, which includes the large scale path loss from one UE to several nearby BSs and some coarse information of the co-channel interference in the system. Based on this information, C\&B estimates the SNR of one UE and its generated INR to nearby BSs, and tries to balance the two. C\&B can be implemented fairly easily, mainly in software. No extra pilots nor the use of backhaul communication is needed in executing C\&B. Further, C\&B can be implemented in a distributed manner with low complexity. Most importantly, C\&B is able to realize the potential benefits promised by CoMP. 
%We propose a novel coordinated open-loop power control scheme, named \emph{Checks and Balances (C\&B)}, which exploits large-scale channel states to select transmission power levels of mobile units, cooperatively across neighboring cells. The key difference from all existing power control schemes is that C\&B explicitly evaluate both impacts of enhancing received signal strength and mitigating co-channel interference, and then balances the tradeoff between the two. Furthermore, the construction of C\&B does not incur any additional cost on pilots, backhaul bandwidth, or signal processing overheads, but only a minimal complexity increase over the industrially standardized non-coordinated solutions. 
%Therefore, C\&B overcomes the common practical issues that prevents existing CoMP techniques from being adopted in real-life applications. 

\item We evaluate the throughput performance of C\&B on an LTE system-level simulation platform, which is carefully calibrated with Huawei. C\&B is shown to provide a $51.9\%$ improvement on the average throughput per cell over the widely adopted Fractional Power Control (FPC) scheme \cite{Whitehead}. In additional comparison with Max Power policy \cite{Furuskar08}, C\&B improves the edge-user throughput
% and power efficiency (Mbits/Joule) 
by $156\%$
% and $5,716\%$, respectively.  
Further, C\&B achieves a per-cell average throughput gain of $21.5\%$ over a reference practical coordinated power control solution named Reverse Link Power Control\cite{Rao07}.  


%\item Verified by system-simulations, C\&B provides a $54.2\%$ improvement on the average cell throughput and a $144\%$ improvement on the edge-user throughput over the existing non-coordinated industry standard power control scheme. Note that the performance gain is obtained solely by C\&B in MAC layer control, no advanced physical layer CoMP technique is involved.
%\item  C\&B is compatible with other CoMP techniques (e.g. CoMP scheduling, physical layer CoMP interference cancellation, beamforming, etc.), such that the throughput can be further improved;
%%\item C\&B novelly builds the direct connection between large-scale path losses and the throughput performance and applies it in power control;
%\item C\&B has low computational complexity, requires no additional control signaling exchange or feedback in backhaul links, compared to existing non-coordinated and coordinated approaches;
%\item The construction of C\&B is universal and adaptive to various cellular system scenarios;
%\item C\&B can be easily implemented on hardware.
%\item C\&B is designed in such a way that it strikes a careful balance between received signal strength and co-channel interference in power control. Our methods have the flavor of cross-layer network control mechanisms, which are rarely exploited in the design of current cellular networks.
\end{itemize}
%The performance comparison is summarized in Table \ref{Table_ResultsSummary}, which presents C\&B's advantages in terms of cell average throughput, cell-edge throughput and power efficiency.



%The rest of the paper is organized as follows. We first introduce the system model in Section \ref{SystemModel}. 
%Next in Section \ref{Principles}, we provide general principles for desirable open-loop power control solution. 
%Next, we present the detailed design of C\&B in Section \ref{Main Design}, followed by system-level simulation results in Section \ref{Simulation}. Finally, we complete our paper with conclusions and future works in Section \ref{Conclusion}. 

\noindent {\bf Related Works:} Non-coordinated power control is standardized in 3GPP protocols \cite{36.213} and has attracted vast research interests \cite{Gipson96, Furuskar08, Whitehead, Castellanos08, Andrews13, Novlan13, Xiao06, Coupechoux11}. There exist three mainstream schemes: (1) Full Compensation Power Control (FCPC) \cite{Gipson96} allocates transmission power to one UE by making full compensation of its large-scale path loss such that all UEs have the same received signal strength, which results in poor performance in per-cell average throughput and inter-cell interference management. (2) Max Power scheme \cite{Furuskar08} let all UEs transmit at their maximum allowable power. It provides high average per-cell throughput, but performs poorly in power efficiency and throughput of UEs at the cell edge. (3) Fractional Power Control (FPC) \cite{Whitehead} is currently the most widely adopted scheme \cite{Andrews13, Novlan13, Xiao06, Coupechoux11}, which allocates transmission power by making fractional compensation of UEs' large-scale path losses, such that UEs in the interior of one cell have stronger received signal strength than UEs at the cell edge. The key drawback remains in the unsatisfying average throughput per cell.
%It greatly outperforms Max Power schemes \cite{Castellanos08} in terms of power efficiency and cell-edge UE throughput, respectively. However, the per-cell throughput performance (though much better than FCPC) remains unsatisfactory. Calibration of FPC to enhance the network performance draws a lot research interests from both theoretical and practical point of views \cite{Andrews13, Novlan13, Xiao06, Coupechoux11}.

Two coordinated power control schemes have been proposed \cite{Rao07, Yang09}, which make additional compensation for large-scale path losses from one UE to its neighboring cells. These schemes are essentially variations of FCPC. Hence, they partially inherit the drawbacks of FCPC which significantly limits the throughput gain. 


==> GlobeCom16_Sumbmission/MainDesign.tex <==
\section{Checks and Balances: A Power Control Design}\label{Main Design}
%The key challenge in open-loop power control is dealing with the tight tradeoff between signal enhancement and co-channel interference mitigation: enhancing signal and mitigating interference respectively require increasing and decreasing transmission power, hence simultaneous improvement can not be achieved. For instance, consider we increase the transmission power of a UE to improve its received SINR and throughput. In the meanwhile, the UE generates stronger interference to nearby cells that degrade the throughput of other UEs. Therefore, overly high or low power assignment both result in decrease of average total throughput per cell (i.e. cell average throughput). And figuring out the proper compromise between signal enhancement and interference mitigation is difficult. Furthermore, the real-life constraints in practical cellular systems make the problem even more challenging.
%
%To take care of the above tradeoff and concerns of universality, robustness, UE-Independence and simplicity, existing approaches (including both coordinated and non-coordinated) decide the transmission power of a UE by applying low-complexity schemes that take into account the large-scale path losses from the UE to different cells. However, never has the SINR-Throughput mapping of the implemented physical layer or its relation with large-scale path losses of a UE been considered. Different from the theoretical Gaussian channel capacity, the SINR-Throughput mapping indicates the system's real achievable spectrum efficiency under various SINR situations. It occurs to us that the possibility of significant improvement on efficiency and fairness lies in these missing parts. Therefore, we propose our coordinated open-loop power control scheme that has the structure shown in Fig. \ref{PC_Structure}.
%\begin{figure}
% \centering \includegraphics[width=3.5in]{PC_Structure.eps} \caption{Structure for Proposed Open-loop Power Control.}
%\label{PC_Structure} \vspace{-0.cm}
%\end{figure}
%Note that the SINR-Throughput mapping is a system \textbf{priori}, thereby acquiring this information does not have any additional cost. 
%
%Now we present our proposed open-loop power control scheme in detail. 

%The task of uplink power control is to make the signal received  at the base station sufficiently strong, and in the meanwhile keep the interference generated to nearby base stations not severe. In practice, overly high and overly low transmission powers are both harmful. Specifically, increasing the transmission power of one UE can increase its  throughput, and meanwhile cause strong interference to nearby cells which will degrade the throughput of other UEs. Hence, there is a tradeoff between signal enhancement (SNR) and interference mitigation (INR). In real systems, it is extremely difficult, if not impossible, to find the optimal tradeoff point between SNR and INR because there are a huge population of users with diverse channel conditions, and channel knowledge is only available for a small amount of local wireless links. So far, there is little success to improve such tradeoff in existing power control approaches. In this section, we propose a power control scheme named checks and Balances (C\&B), which approximately evaluates the impacts of both SNR and INR in order to select the proper transmission power that balances their tradeoff.


%In this section, we propose a power control scheme called checks and Balances (C\&B). Different from existing power control approaches, C\&B has utilized large-scale path losses to nearby cells, the interference level measured at each cell, and the throughput performance of physical layer to determine the transmission power, and achieve a high throughput gain.
%
%It is worth emphasizing that the SINR-throughput mapping $T(SINR)$ is a system priori and can be easily achieved by the power controller with only a one-time forward from the AMC module. However, it has not been used by any existing open-loop power control approach (refer to Fig. \ref{OLPC}). With this inspiration, we take $T(SINR)$ into account for our proposed power control scheme which has the construction structure as shown in Fig.\ref{C&B_Structure}. This makes our scheme essentially different from all existing approaches and gives us the chance to build the direct connection between large-scale path losses and realistic throughput performance in power control design. 
%\begin{figure}
% \centering \includegraphics[width=2in]{C&B_Structure.eps} \caption{Construction of our proposed power control.}
%\label{C&B_Structure} \vspace{-0.cm}
%\end{figure}
%
%%\subsection{Scheme Design}
%The proposed power control scheme is named \emph{Checks and Balances (C\&B)}. The key idea of C\&B is to
% \begin{itemize}
% \item \emph{\textbf{Checks}} UEs' received signal strength (i.e. SNR) and generated interference (i.e. INR) to nearby cells;
% \item \emph{\textbf{Balances}} the tradeoff between the two. 
% \end{itemize}
% Thus, C\&B is capable of explicitly adjusting the balance on the tradeoff between enhancing received signal strength and mitigating inter-cell interference. To guarantee the practicality, we make the execution of C\&B universal and adaptive to different cellular system scenarios. The power allocation process is UE-specific and operated independently by each cell, which has the same pattern as existing power control schemes. Besides seeking throughput improvement, we let the computational complexity and implementation requirement remain low so that C\&B can be readily adopted in practice. The detailed C\&B scheme is constructed in following steps. 

%\subsection{Preliminary: Large-scale Modeling} \label{Preliminary}
%Consider UE $u_k$ transmits to cell $c_k$ with power $P_k$ and interferes its nearby cell $c_j$ ($\forall j \neq k$), $c_k$ can calculate  $u_k$'s received SNR and generated INR as:
%%$u_k$'s received large-scale Signal-to-Noise Ratio (SNR), Signal-to-Interference-plus-Noise Ratio (SINR), Interference-over-Thermal (IoT) at its serving cell $c_k$, and generated large-scale Interference-to-Noise Ratio (INR) to its neighboring cell $c_j$ can be calculated as below:
%\begin{eqnarray}
%SNR(P_k) &=& \frac{PL_{kk}^{-1} \cdot P_k}{N_0}, \label{Eq_SNR} \\
%%SINR_k &=& \frac{PL_{kk}^{-1} \cdot P_k}{N_0 + \sum_{j \neq k}{P_j \cdot PL_{jk}^{-1}}}, \label{Eq_SINR} \\
%%IoT_k &=& \frac{N_0 + \sum_{j \neq k}{P_j \cdot PL_{jk}^{-1}}}{N_0}, \label{Eq_IoT} \\
%INR_{kj}(P_k) &=& \frac{PL_{kj}^{-1} \cdot P_k}{N_0}, \label{Eq_INR} 
%\end{eqnarray}
%where $N_0$ denotes the average noise power, which is assumed to be the same and known for all UEs. 
%%Note that only large-scale path loss is taken into account due to its availability in open-loop power control, as shown in Fig. \ref{OLPC} and Fig. \ref{C&B_Structure}.  
%
%A widely adopted metric named interference over thermal noise (IoT) is defined as the ratio of UE's received interference-plus-noise power over noise power. Let the transmission power of UE $u_j$ that served in cell $c_j$ and its associated large-scale path loss to cell $c_k$ be $P_j$ and $PL_{jk}$ respectively, the received IoT for UE $u_k$ can be expressed as:
%\begin{eqnarray}
%IoT_k = \frac{N_0 + \sum_{j \neq k}{P_j \cdot PL_{jk}^{-1}}}{N_0}, \label{Eq_IoT} 
%\end{eqnarray} 
%However, neither $P_j$ nor $P_{jk}$ is known to cell $c_k$ in the process of power control. This makes it impossible in practice for cell $c_k$ to calculate $IoT_k$ or the received SNR of $u_j$, i.e. $SNR(P_j)$. Therefore, we need to parameterize these metrics in our design of C\&B. 
%
%At last, the received SINR of UE $u_k$ can be expressed as:
%\begin{eqnarray}
%SINR_k = \frac{SNR(P_k)}{IoT_k} \label{Eq_SINR}
%\end{eqnarray}
%All above large-scale metrics are widely used in existing power control approaches, especially in the associated parameter selection. In our C\&B design, we make use of these metrics from a different point of view.

In this section, we present a novel power controller design, called Checks and balances (C\&B),  for uplink cellular systems. This power controller requires very little information, including the throughput versus SINR curve of the receiver design, the large-scale path loss from one UE to several nearby BSs, and some coarse distribution information of the co-channel interference in the cellular system. The key idea in C\&B is to cooperatively balance the SNR of a UE and its generated INR to nearby BSs. The complexity of C\&B is very low, and the throughput gain is huge. One can consider C\&B as the simplest implementation of CoMP, which provides significant throughput improvement without incurring huge cost in pilots or backhaul. There is no upgrade of the physical layer design, except for the change of uplink transmission power.

\subsection{Approximations of SINR and Throughput}
% The SINR-Throughput mapping is based on the implemented adaptive modulation and coding (AMC) module, available modulation and coding scheme (MCS) options and adopted estimation/detection/receiver techniques. In real-life cellular system, the AMC module assigns proper MCS to the scheduled UE according to its cumulative SINR estimation and SINR prediction, thereby greatly decide the final throughput performance. Fig. \ref{AMC_All} illustrates a sample SINR-Throughput mapping that we implement in our system-level simulation platform. It reflects the spectrum efficiency performance upper bound of given system physical layer in the ideal scenario. In practice, the real spectrum efficiency becomes even worse due to real-life constraint, e.g. delay of control signaling, estimation error. We can see the huge gap between achievable spectrum efficiency and Gaussian channel capacity, which implies that it is more practical to get SINR-Throughput mapping,other than theoretical capacity, involved in power control. 
%Recall that the SINR-Throughput mapping represents the best achievable spectrum efficiency under given SINR, as shown in Fig. \ref{SINR-Throughput Mapping}. 
C\&B can operate in the open-loop mode, when only large scale CSI is utilized, whereas small scale CSI is unavailable due to the lack of instantaneous channel estimation pilot. The large-scale path loss between UE $u_j$ and cell $c$ is defined as: 
\begin{eqnarray}
\text{PL}_j \triangleq \mathbb{E}\big[|h_j|^2\big]^{-1},  \label{PL}
\end{eqnarray} 
where $\mathbb{E}[\cdot]$ denotes the expectation. When we only consider such large-scale path losses, $u$'s received signal-to-noise ratio (SNR) and interference over thermal noise (IoT) at $c$, and generated interference-to-noise ratio (INR) to $c_j$ can be respectively approximated as:
\begin{eqnarray}
\text{SNR}(P) &=& \frac{\text{PL}^{-1} \cdot P}{N_0}, \label{Eq_SNR} \\
\text{IoT} &=& \frac{N_0 + \sum_{j}{P_j \cdot \text{PL}_{j}^{-1}}}{N_0}, \label{Eq_IoT}\\
\text{INR}_{j}(P) &=& \frac{\text{PL}_{u \to j}^{-1} \cdot P}{N_0}, \label{Eq_INR} 
\end{eqnarray}
where $N_0$ denotes the average noise power and is assumed to be the same and known for all UEs. We also define $\text{PL}_{u \to j}$ as the large-scale path loss from UE $u$ to cell $c_j$. Derived from Eq. (\ref{Eq_SNR}) and (\ref{Eq_IoT}), we can approximate the received SINR of UE $u$ as:
\begin{eqnarray}
\text{SINR} = \frac{\text{SNR}(P)}{\text{IoT}}. \label{Eq_SINR}
\end{eqnarray}


%The SINR-Throughput mapping is system priori knowledge which can be achieved with no extra cost. In order to avoid the exhaustive search incurred by directly implementing the abnormal stair-shaped $T(SINR)$ and relax the associated hard transitioning effect due to switching MCSs, we introduce a piece-wise function $f(SINR)$ for approximation:
As C\&B only acquires large scale CSI and approximated SINR information, there is no need to use an accurate throughput curve to determine the transmission power. Therefore, we introduce a piece-wise function to approximate the foregoing throughput curve:
\begin{eqnarray}\label{U_Basic}
%f(\theta) = \left\{\begin{array}{l l} 0,&\text{ if } \theta<\theta_{min};\\
%g(\theta),& \text{ if } \theta_{min} \leq \theta \leq \theta_{max};\\
%g(\theta_{max}),& \text{ if } \theta > \theta_{max}.
%\end{array}\right.
f(\text{SINR}) = \min\big[T_{\max}, a\cdot \log_2(1+b\cdot \text{SINR})\big],
\end{eqnarray}
%where $g(SINR)$ is a monotonically increasing smooth function. In the paper, we set $g(SINR)$ as:
%\begin{eqnarray}
%g(SINR) = a\cdot \log_2(1+b\cdot SINR)
%\end{eqnarray}
where $T_{\max} = 4.18$, $a = 0.7035$ and $b = 0.7041$. These parameters are achieved by curve fitting as shown in Fig. \ref{AMC_Approximation}. Note that for different physical layer designs, we can always find such an approximated throughput function $f(\text{SINR})$. Next, we use function $f(\text{SINR})$ to evaluate the throughput of one UE $u$ and the throughput of the UEs interfered by UE $u$.
%$\theta_{min}$ and $\theta_{max}$ denote the SINR value at which $f(\theta)$ achieves minimum and maximum, respectively. We set these parameter values at: $\theta_{min} = -10$ dB, $\theta_{max} = 19.5$ dB. 
%One can select alternative forms of $f(SINR)$ based on different SINR-Throughput mapping situations. Note that $f(SINR)$ is upper bounded by the maximum of $T(SINR)$, as illustrated in Fig. \ref{AMC_Approximation}. We let $f(SINR)$ serve as the basic function for evaluating the utilities of one UE's received SNR and generated INR.
\begin{figure}
 \centering \includegraphics[width=2in]{figs/AMC_Approximate.eps} \caption{Throughput Curve Approximation.}
\label{AMC_Approximation} \vspace{-0.2cm}
\end{figure}


\subsection{Checking the Influence of SNR and INR} \label{SNR Utility}
Consider an arbitrarily chosen UE $u$, its uplink throughput can be approximated as 
\begin{eqnarray}
U_S(P) = f\left(\frac{\text{SNR}(P)}{\text{IoT}_{S}}\right), \label{U_SNR}
\end{eqnarray}
where $\text{IoT}_S$ denotes a prior estimation of the interference experienced by UE $u$. Note that the interference that UE $u$ will experience during its transmissions are not available to the power controller, since transmission of such information requires communication throughput backhaul links which is prohibited in the open-loop mode. Hence, we propose a method to estimate $\text{IoT}_S$. 
%In the simulation environment described in Section \ref{Simulation}, the distribution of the interference over thermal noise ratio in the uplink cellular system is illustrated in Fig. \ref{SNR_vs_IoT}. 
We select  $\text{IoT}_S$ to be the $95^{th}$ percentile of IoT that experienced by an arbitrary UE, which is $\text{IoT}_S=9$ dB. Note that this statistical distribution can be collected at the BS. In practical applications, we recommend to initialize the system with this value and update it according to the measured IoT distribution. The approximated throughput $U_S(P)$ is plotted in Fig. \ref{Sample_Utility_SNR}, which increases with the transmission power $P$.
%\begin{figure}
% \centering \includegraphics[width=2in]{figs/SNR_vs_IoT.eps} \caption{Time-average SNR and IoT distributions.}
%\label{SNR_vs_IoT} \vspace{-0.2cm}
%\end{figure}


%where we introduce parameter $IoT_{S}$ to denote the received IoT.

%We set $IoT_S$ at the same value for all UEs to keep low implementation complexity. In order to take the influence of severely strong interference into account, we select it as the $95^{th}$ percentile of instantaneous IoT that experienced by an arbitrary UE. Note that the instantaneous IoT can be measured and accumulated at the receiver of each cell. Achieved by multiple rounds of our simulations, the parameters is chosen as $IoT_{S} = 9$ dB. In practical applications, we recommend to initialize the system with this selection and update it according to the realistic instantaneous IoT distribution of an arbitrary UE, which can be generated after a training process. 

%The utility $U_S(P_k)$ increases with enhancing transmission power as presented in Fig. \ref{Sample_Utility_SNR}, which indicates the benefit in received signal enhancement. Hence, the desire for strong received signal motivates power increase.
\noindent
\begin{figure*}[htp!]
\vspace{-0.2in}
\centerline{
\subfloat[Approximated throughput of UE u.]
{\includegraphics[width=2.1in]{figs/Utility_SNR_Linear.eps}
\label{Sample_Utility_SNR}}
\subfloat[Approximated total throughput of UEs that are interfered by UE $u$.]
{\includegraphics[width=2.1in]{figs/Utility_INR_Linear.eps}
\label{Sample_Utility_INR}}
\subfloat[Weighted sum throughput approximation.]
{\includegraphics[width=2.1in]{figs/Utility_WeightedSum_Linear.eps}
\label{Sample_Utility_Sum}}
}
%\vspace{-0.1in}
\caption{Approximated throughput functions for C\&B power controller design.}
\vspace{-0.2in}
\end{figure*}

%\begin{figure}
% \centering \includegraphics[width=2.5in]{Utility_SNR_Linear.eps} \caption{Utility of received SNR $U_S(P_k)$ vs. transmission power $P_k$ of a sample UE $u_k$.}
%\label{Sample_Utility_SNR} \vspace{-0.cm}
%\end{figure}

Consider the UEs that are notably interfered by UE $u$, their sum uplink throughput can be approximated as: 
\begin{eqnarray}
U_I(P) = \sum_{\text{PL}_{u \to j} < \text{PL}_{th}} f\bigg(\frac{\text{SNR}_I}{\text{IoT}_I + \text{INR}_{j}(P)}\bigg).   \label{U_INR}
\end{eqnarray}
Note that we only consider the non-negligible interference generated by UE $u$. To this end, we set $\text{PL}_{th}$ as the path loss such that $u$ with maximum allowable transmission power $P_{\max}$ can generate interference that is stronger than noise, i.e.,
\begin{eqnarray}
\frac{\text{PL}_{th}^{-1} \cdot P_{\max}}{N_0} > 1, \label{Eq_PLth} 
\end{eqnarray}
where $P_{\max} = 200$ mW ($23$ dBm) \cite{3GPP25.996}. Furthermore, these UEs' transmission power and received interference are unknown to the power controller of UE $u$ in the open-loop mode due to the prohibition of communication via backhaul links. Therefore, we also propose methods for estimating parameters $\text{SNR}_I$ and $\text{IoT}_I$, which denotes the received SNR and IoT (excluding the interference generated by $u$) of UE that served in cell $c_j$, respectively. These parameters are computed by using physical layer SINR region [$-6.5$ dB, $17$ dB], the details  will be explained in the journal version.
%Similarly as selecting $\text{IoT}_S$, we choose $\text{IoT}_I$ to be the $75^{th}$ percentile of IoT that experienced by an arbitrary UE, which is $\text{IoT}_I=5$ dB. The distribution of the SNR in the uplink cellular system is illustrated in Fig. \ref{SNR_vs_IoT}. $\text{SNR}_I$ is selected to be the $95^{th}$ percentile of IoT that experienced by an arbitrary UE, which is $\text{SNR}_I=24$ dB.

%Since UEs with high SNR are less vulnerable to interference, we choose $SNR_I$ as the $70^{th}$ percentile of instantaneous received SNR for an arbitrary UE. $IoT_I$ is chosen to be the $75^{th}$ percentile of instantaneous IoT experience by an arbitrary UE, which is lower than $IoT_S$ because it does not include the interference from UE $u_k$. Also achieved by multiple test rounds of simulation, $SNR_I $ and $IoT_I$ are set as $24$ dB and $5$ dB, respectively. 
%$INR_{kj}(P_k)$ and $INR_{kj}(P_{sat})$ are the large-scale INR that $u_k$ interferes cell $c_j$ at transmission power $P_k$ and $P_{sat}$, calculated as in Eq. (\ref{Eq_INR}). We will discuss the saturated power $P_{sat}$ later. $INR_{th}$ denotes the non-negligible INR threshold that is set as $inr_th = 0$ dB, i.e. 
The approximated sum throughput $U_I(P)$ is plotted in Fig. \ref{Sample_Utility_INR}, which decreases with the transmission power $P$.
%Fig. \ref{Sample_Utility_INR} shows that $U_I(P_k)$ decreases as $P_k$ increases, which implies the potential throughput loss due to stronger interference that generated by $u_k$. Therefore, demand in interference mitigation leads to transmission power decrease. 
%\begin{figure}
% \centering \includegraphics[width=2.5in]{Utility_INR_Linear.eps} \caption{Utility of generated INR $U_I(P_k)$ vs. transmission power $P_k$ of a sample UE $u_k$.}
%\label{Sample_Utility_INR} \vspace{-0.cm}
%\end{figure}

%\begin{figure}
% \centering \includegraphics[width=2.5in]{Utility_WeightedSum_Linear.eps} \caption{Weighted sum utility $U_{w-sum}(P_k)$ vs. transmission power $P_k$ of a sample UE $u_k$.}
%\label{Sample_Utility_Sum} \vspace{-0.cm}
%\end{figure}

\subsection{Balancing the Two} 
%Enlarging $U_S(P_k)$ and $U_I(P_k)$ respectively leads to transmission power increase and reduction, which indicates the tight tradeoff between enhancing received signal and mitigating inter-cell interference. In order to find out the proper balance of such tradeoff, we introduce the weighted sum utility which can be maximized by appropriately select the transmission power:
%\begin{eqnarray}
%U_S(P_k) + \zeta \cdot U_I(P_k)   \label{U_sum}
%\end{eqnarray}
%where $\zeta$ is the weight parameter that adjusts the relative importance between SNR utility and INR utility, and is set at $1.1$. As presented in Fig. \ref{Sample_Utility_Sum}, the weighted sum utility is maximized at a unique transmission power, i.e. the balance we choose based on the overall benefit for both received signal enhancement and inter-cell interference mitigation. Hence, we aim to solve the following problem:
In order to find a proper balance between SNR and INR, we consider the following weighted sum throughput maximization problem:
\begin{eqnarray}
\max_{0 \leq P \leq P_{\max}} U_S(P) + \zeta \cdot U_I(P), \label{U_Maximize}
\end{eqnarray}
%where $P_{low}$ and $P_{sat}$ are the lower bound and saturated value of transmission power, defined as: $P_{low} = \min(P_{max},P_{low}')$, $P_{sat} = \min(P_{max},P_{sat}')$. $P_{max} = 23$ (dBm), is the maximum transmission power constraint. $P_{low}'$ and $P_{sat}'$ denote the transmission power at which we have $SNR(P_{low}') = SNR_{low}$ and $SNR(P_{sat}') = SNR_{sat}$, respectively. We select $SNR_{low} = 5$ dB and $SNR_{sat} = 27$ dB. 
where $\zeta$ is the weight parameter that adjusts the relative importance of SNR and INR, which is chosen around $1$. Large $\zeta$ (e.g. $\zeta>1$) indicates more focus on mitigating INR rather than enhancing SNR, which leads to more conservative transmission power. This benefits the UEs with poor channel states due to the reduced interference, while constraining the transmission power of UEs with good channel states that prevents them from achieving better throughput. It works the other way around when we choose small $\zeta$ (e.g. $\zeta <1$). Tending to suppress strong interference, we initially select $\zeta$ to be $1.3$. As shown in Fig. \ref{Sample_Utility_Sum}, the weighted sum throughput is maximized at a unique transmission power, i.e., the balance we choose between SNR and INR. 
%As presented in Fig. \ref{Sample_Utility_Sum}, the weighted sum utility is maximized at a unique transmission power, i.e. the balance we choose based on the overall benefit for both received signal enhancement and inter-cell interference mitigation. Such power can be selected for each UE in a distributed manner, since the only the large-scale path losses from one UE to its serving and neighboring cells are required.

\IncMargin{1em}
\begin{algorithm}[h]
\SetKwFunction{CandidateUser}{CandidateUser}
\SetKwData{NULL}{NULL}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}

 \textbf{Given} $l= -10$ dBm, $r = P_{\max}$ , \text{tolerance} $\epsilon=0.1$\;
\uIf{$r-l < \epsilon$} {
$m:= P_{\max}$;
}
\Else{ 
 \While{$r-l \geq \epsilon$}{
   
       $m:= (l+r)/2$\;
       \uIf{$U_S'(m) + \zeta \cdot U_I'(m)< 0$}{
       $l:=m$; 
       }
       \Else{ 
      $r:=m$;
      }
    }
}
 
 
\Return{$P:=m$.} 
 
\caption{Bisection method for solving (\ref{Gradient_0}) .}\label{alg_Bisection}
\end{algorithm}
\vspace{-0.2in}
\DecMargin{1em}

It is easy to show that Problem (\ref{U_Maximize}) is a one-dimensional quasi-convex optimization problem, and thereby can be obtained by solving the following problem:
\begin{eqnarray}
U_S'(P) + \zeta \cdot U_I'(P)= 0. \label{Gradient_0}
\end{eqnarray}
%In order to quickly locate the solution,  we apply a bisection search method, as shown in {\bf Algorithm \ref{alg_Bisection}}.
We use bisection method to find the solution of (\ref{Gradient_0}), with the detailed steps presented in Algorithm \ref{alg_Bisection}. This algorithm is easy to implement on DSP, and the number
of iterations for convergence is less than 10. We note that Algorithm 1 is a fully distributed algorithm, where each UE can choose its transmission power independently.

%This algorithm is easy to implement on either hardware or DSP, and the number of needed iterations for convergence is less than $10$.

%Note that the construction of C\&B is universal and adaptive to different cellular system scenarios. The power allocation process is UE-specific and independent from other UEs/cells. The computational complexity and implementation requirement remain low. It is obvious that the selection of parameters is a critical part of C\&B, which is discussed in detail in the next subsection.

%\subsection{Guidelines for Parameter Selection}\label{Parameter Selection}
%According to the given adopted physical layer techniques, cellular network deployment, UE density/mobility, the associated parameters can be easily adapted by following a universal approach. The key idea is to select the parameter values based on their physical meanings from definition.

%First, we decide the desirable SINR range $[\theta_{low},\theta_{sat}]$. Recall the definition of $f(\theta)$ in (\ref{U_Basic}), increasing SINR over $\theta_{max}$ does not provide additional benefit. Hence, we set the saturated SINR as $\theta_{sat} = \theta_{max}$. On the other hand, the achievable spectrum efficiency is undesirably low (marginally greater than zero) with SINR below 0 dB, as shown in Fig. \ref{AMC_Approximation}. Therefore, we set a lower bound for desirable SINR at $\theta_{low} = 0$ dB. We aim to let the average SINR of almost all UEs lies the desirable SINR range after power control.
%
%Second, we pick the value for the weight parameter $\zeta$. As $\zeta$ increases, we focus more on reducing interference other than boosting received signal strength, and vice versa. It is chosen around the value $1$, based on the given cellular system circumstance (e.g. UE density, cell size, urban/suburban area, etc.).  
%
%Third, we select the IoT range $[IoT_{\min},IoT_{\max}]$. $IoT_{min}$ and $IoT_{max}$ are chosen to be the $10^{th}$ and $90^{th}$ percentile of instant IoT that experienced by an arbitrary UE. Achieved by our training process of simulations, the parameters are set as $IoT_{\min} = 2$ dB and $IoT_{\max} = 6$ dB. In practical situations, we recommend to initialize the system with these selections and update them according to the realistic instant IoT distribution of an arbitrary UE, which can be generated after a training process.
% with an acceptable protection interval $\sigma$. Low IoT indicates good interference management. $[iot_{\min},iot_{\max}]$ sets the objective UEs' average IoT range result after power control. To overcome the unpredictable circumstance variations in the cellular system, we introduce protection interval $\sigma$, which is chosen between $1.2$ (i.e. 1 dB) and $2$ (i.e. 3 dB). Consider the resulting average IoT arrange to be $[iot'_{min},iot'_{max}]$, it is regarded as acceptable if: $\frac{iot_{\min}}{\sigma} \leq iot'_{\min} \leq iot_{\min}\cdot \sigma$, and $\frac{iot_{\max}}{\sigma} \leq iot'_{\max} \leq iot_{\max}\cdot \sigma$. Otherwise, we adjust the values of $iot_{min}$ and $iot_{max}$. In other words, the desirable average IoT range can be selected iteratively by running training process.

%Fourth, we choose the desirable SNR range $[SNR_{low},SNR_{sat}]$. The objective is to make the SINR of an arbitrary UE lies in the desirable SINR range with the instant IoT range taken into account. To further guarantee it, we introduce a protection parameter $\sigma = 3$ dB, and set $SNR_{sat} = \theta_{sat} + IoT_{max} + \sigma$, $SNR_{low} = \theta_{low} + IoT_{\min} + \sigma$. 
%
%At last, we set the rest parameters according to all the above parameter selections. IoT parameters are selected as: $IoT_S = IoT_{max} + \sigma$, $IoT_I = IoT_{\min} + \sigma$. For all UEs, we choose $SNR_I = \frac{SNR_{low} + SNR_{sat}}{2}$. 
%
%It is important to see that C\&B is a novel power control scheme that essentially different from all existing non-coordinated and coordinated approaches. The key differences are taking  the SINR-Throughput mapping into account, building the direct connection between throughput and large-scale path losses, and explicitly adjusting the balance on the tradeoff between signal enhancement and interference mitigation. In the following, we verify that these differences make C\&B significantly outperforms existing power control schemes.


==> GlobeCom16_Sumbmission/Principles.tex <==
\section{Challenges of Practical Power Control}\label{Principles}

%The objective of open-loop power control is to adjust UEs' transmission power, such that strong enough received signal is guaranteed and severe co-channel interference is avoided. Moreover, the construction of power control is subject to a number of constraints in real-life cellular systems, e.g. huge number of involved cells, complicated environment circumstances, numerous UEs with various mobility, etc. Therefore, it requires open-loop power control to have following properties:
The task of uplink power control is to determine the transmission power of each UE, such that the signal received  at the base station is sufficiently strong, and the interference generated to nearby base stations is not severe. In reality, this task is arduous because of many factors, such as enormous users and cells, complicated propagation environment, and dynamic user mobility. These factors impose the following requirements in the design of uplink power control:
\begin{itemize}
\item \textbf{Efficient:} High throughput is required to meet the requirement of cellular systems.
%High throughput is provided to satisfy the communication speed requirements of current (e.g. 3G, LTE) and next generation (e.g. 5G, 6G) cellular systems.

\item \textbf{Reliable:} The channel condition and interference power may vary acutely over time. For example, a strong interference source may exist in one slot and disappear in the next slot because of dynamic scheduling. The quality of service is required be sufficiently high in such scenarios.

\item \textbf{Fair:} The uplink throughput varies from one UE to another, which can be quite low for UEs with poor channel conditions. The power controller needs to reduce the interference level such that the  5-percentile throughput, which is usually termed cell-edge throughput, is sufficiently high.
%Guarantee acceptable performance for UEs that have poor channel and/or confront strong interference. The throughput of these UEs, measured by $5$ percentile throughput (i.e. $5\%$-Edge throughput), is greatly lower than the average and indicates the fairness among UEs.

\item \textbf{Autonomic:} UEs' power allocation within once cell is decided independently from UEs in other cells. No assistance from other UEs/cells, control signaling exchange/iterations with other power control modules, or feedback is needed.

%\item \textbf{Simple:} The computational and implementational complexity is low. UEs' connection establishment process is simplified, performance analysis and adaptive adjustment can easy to be made.

\item \textbf{Universal:} The power control algorithm must be universally applicable in all system circumstances, which differ in cell size, UE density, mobility speed, and path loss factor.
\end{itemize}

In practice, overly high and overly low transmission powers are both harmful. Specifically, increasing the transmission power of one UE can increase its  throughput, and meanwhile cause strong interference to nearby cells which will degrade the throughput of other UEs. Hence, there is a tradeoff between signal enhancement (SNR) and interference mitigation (INR). In real systems, it is extremely difficult, if not impossible, to find the optimal tradeoff point between SNR and INR because there are a huge population of users with diverse channel conditions, and channel knowledge is only available for a small amount of local wireless links. Existing power control algorithms \cite{Whitehead}-\cite{Rao07} usually determine the transmission power based on a simple heuristic linear equation with one or two parameters, and explore different tradeoff points by adjusting these parameters. So far, there is little success to improve these algorithms, because of the complicated tradeoff between SNR and INR and the practical requirements mentioned above. 
%All of the above requirements are crucial to a desirable open-loop power control solution. Universality and robustness together decide whether the proposed solution can be widely adopted. Efficiency and fairness guarantee the designed scheme to satisfy diverse quality of service (QoS) requirements. UE-Independence and Simplicity lead a open-loop power control scheme to be implemented in practical systems due to the low investment cost and infrastructure requirement. 
In the following section, we propose our open-loop power control scheme that has all these valuable properties. 


==> GlobeCom16_Sumbmission/Simulation.tex <==
\section{Performance Evaluation on System-level Simulation Platform}\label{Simulation}
%In this section, we present C\&B's advantages over FPC, Max Power and coordinated Reverse Link Power Control schemes by calibrated system-level simulations.

\subsection{Simulation Platform Configuration}
We consider an LTE uplink cellular network \cite{36.814}, where the BSs are located on
a typical hexagonal lattice including $19$ BS sites, $3$ sectors per site. Each sector is regarded as a cell. The minimal distance between two neighboring sites is 500 meters (Macrocell) \cite{36.814}. The UEs are uniformly distributed in the entire network area. The distance from a UE to a nearest BS is no smaller than 35 meters \cite{3GPP25.996}. Each UE has a single antenna, and the BSs are equipped with 2 antennas per sector. The wireless channel coefficients and BS antenna pattern are generated by following the SCM model for Urban Macro environments in 3GPP TR 25.996 \cite{3GPP25.996}, where 3D antenna pattern and Rayleigh fading \cite{Zheng03} are adopted. We set the maximum doppler shift frequency at $7$ Hz according to moving speed $3$ km/h and carrier frequency $2.5$ GHz. The receivers employ non-CoMP maximum mean square error (MMSE) estimation \cite{Tse05} with interference rejection combination (IRC) techniques \cite{Leost12}. To obtain the channel coefficients, we estimate the pilots, i.e. demodulation reference signals (DMRS) \cite{36.213}, with DFT-based estimation \cite{Huang10}. 
%This guarantees that all throughput gain is because of our novel MAC-layer design, without any contribution from physical-layer CoMP techniques. 
Adaptive Transmission Bandwidth (ATB) \cite{ATB} non-CoMP packet scheduling scheme is implemented. The frequency bandwidth is 10MHz, and the noise figure of each BS receiver is 5 dB \cite{36.213}.
%The UEs may choose from $29$ allowable MCSs with the transport block size mapping specified in \cite[Section 7.1.7]{36.213}. The MCS of each UE is determined by the AMC module which sets the target BLER at $10\%$.  
We set a uniform penetration loss of $20$ dB \cite{3GPP25.996} for all users. 
The delay of control signaling is uniformly set as $6$ ms (i.e. 6 time slots) \cite{36.321}. The wrap around technique is employed to avoid the border effect. The parameters of our system level simulation platform are listed in Table \ref{tab2}.

We use the proportional-fair (PF) policy \cite{Tse05} in stochastic network control in which we schedule the UEs to maximize the following function at each time slot:
\begin{eqnarray}
\sum_{u} \frac{(r_u[t])^\alpha}{(\bar{r}_u)^\beta},  \label{PF_eq}
\end{eqnarray}
where $r_u[t]$ and $\bar{r}_u$ denote the UE $u$'s potentially achieved data rate in time slot $t$ and long-term average data rate, respectively. We set the two associated parameters at: $\alpha =1$, $\beta = 1$. 

We compare C\&B with three reference policies: One policy is the widely used fractional power control (FPC) scheme, which determines the transmission power $P^{FPC}$ of UE $u$ for each resource block by \cite{36.213}:
\begin{eqnarray}
P^{FPC} = \min(P_{\max}, P_0^{FPC} + \kappa \cdot \text{PL}),   \label{FPC_eq}
\end{eqnarray}
where $P_{\max}$ is the maximum power constraint, $P_0^{FPC}$ is the default transmission power, and $\text{PL}$ is the large-scale path loss from UE $u$ to its serving cell. The values of the parameters are $P_{\max} = 23$ dBm, $P_0^{FPC} = -87$ dBm and $\kappa = 0.8$. The second policy is Max Power, which sets all UEs at their maximum allowable transmission power $P_{\max}$. The third reference policy is the coordinated Reverse Link Power Control (RLPC) scheme, where the transmission power $P^{RL}$ is decided by \cite{Rao07}:
\begin{eqnarray}
P^{RL} = \min\big(P_{\max}, P_0^{RL} + \phi \cdot \text{PL} + (1-\phi) \cdot \text{PL}_{\min} \big),   \label{RLPC_eq}
\end{eqnarray}
where $\text{PL}_{\min}$ denotes the minimum path loss from $u$ to its neighboring cells. The rest parameters are selected as $P_0^{RL} = -102$ dBm and $\phi = 0.8$. The parameters of C\&B are chosen as we discussed in Section \ref{Main Design}.


\begin{table}

\centering
\caption{SYSTEM LEVEL SIMULATION PARAMETERS}\label{tab2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l}
 \hline
Parameter& Setting\\ 
\hline
Deployment Scenario & 19 BS sites, 3 sectors (cells) per site, \\
&wrap-around \\
Inter-site Distance & 500m (Macrocell)\\
System Bandwidth & 10MHz [50 PRBs, 2 used for control] \\
Avg. UEs per Cell & 10\\
UE/BS Antennas & 1/2 per cell\\
Distance-dependent Path Loss& According to 3GPP 36.814 \cite{36.814}\\
Shadowing Standard Deviation & 8 dB \\
Antenna Pattern & 3D\\
Penetration Loss & 20 dB\\
Scheduling Decision Delay & $6$ ms\\
Target BLER & $10\%$\\
Traffic Model & Fully backlogged queues \\
%&Random packet arrivals\\
Scheduling Algorithm & ATB\\
Power Control (PC) scheme & FPC, Max Power, RLPC, C\&B \\
Stochastic Network Control Scheme & Proportional Fair (PF)\\
%&Closed-loop power adjustment\\
%$\alpha$ (for PC) & 3.5\\
%$\beta$ (for PC) & 25 dB\\
%$\zeta$(for PC) & 5dB\\
%$P_0$ (for FPC) & -85 dBm\\
Link Adaptation & AMC, based on 3GPP TS 36.213 \cite{36.213}\\
BS Receiver Type & IRC MMSE\\
Channel Estimation & DFT-based Estimation\\
Maximum Doppler Shift & 7Hz \\
$\alpha$ (PF) & 1\\
$\beta$ (PF) & 1\\
$P_{\max}$ & $23$ dBm\\
$P_0^{FPC}$ (FPC)& $-87$ dBm\\
$\kappa$ (FPC)& 0.8 \\
$P_0^{RL}$ (RLPC) & $-102$ dBm\\
$\phi$ (RLPC) & 0.8\\
 \hline
\end{tabular}
}
\vspace{-0.2in}
\end{table}

\subsection{Simulation Results}
We compare the performance of different power control schemes in terms of three key metrics: cell average throughput (i.e. sum average throughput per cell), cell edge throughput and power efficiency. In particular, cell edge throughput is defined as the $5^{th}$ percentile of average throughput among all UEs, denoted as $5\%$-Edge, which is widely used in evaluating the performance of UE fairness \cite{Furuskar08,Castellanos08,Coupechoux11}.
\noindent
\begin{figure*}[htp!]
\vspace{-0.1in}
\centerline{
\subfloat[Time-average received SNR.]
{\includegraphics[width=2in]{figs/SNR_500m_7Hz.eps}
\label{SNR_500m_7Hz}}
\subfloat[Time-average experienced IoT.]
{\includegraphics[width=2in]{figs/IoT_500m_7Hz.eps}
\label{IoT_500m_7Hz}}
\subfloat[Time-average throughput.]
{\includegraphics[width=2in]{figs/Throughput_500m_7Hz.eps}
\label{Throughput_500m_7Hz}}
%\subfloat[Time-average power efficiency.]
%{\includegraphics[width=2in]{PowerEfficiency_500m_7Hz.eps}
%\label{PowerEfficiency_500m_7Hz}}
}
%\vspace{-0.1in}
\caption{Simulation results in Macrocell scenario.}
\vspace{-0.2in}
\end{figure*}

\subsubsection{Performance Comparison in Macrocell Scenario}
First, we investigate the performance in enhancing received signal strength, which is evaluated by time-average SNR as illustrated in Fig. \ref{SNR_500m_7Hz}. It can be seen that C\&B, with the weight parameter set as $\zeta = 1.3$, is able to significantly boost UEs' time-average SNR over FPC. Particularly, more than $40\%$ UEs have gained at least $3.5$ dB and approximately $20\%$ UEs  even achieve more than $10$ dB SNR increase. C\&B also improves the SNR of the top $20\%$ UEs compared to RLPC, which greatly benefit the UEs with good channel conditions. It is clear that Max Power has the best SNR performance due to the maximum transmission power. Nevertheless, it simultaneously incurs severe interference which is quite undesirable.

Next, we switch our attention on the interference mitigation performance, which is represented by the time-average IoT as shown in Fig. \ref{IoT_500m_7Hz}. Compared with FPC, C\&B only slightly increase the UEs' average IoT by $1.5$ dB. On the other hand, C\&B performs a lot better than Max Power and shows clear advantage over RLPC in suppressing the inter-cell interference.

Now we concentrate on the throughput performance, which is the comprehensive result of signal enhancement and interference mitigation. In comparison with FPC and RLPC,  C\&B noticeably improves the throughput of UEs with good channel condition (the top $30\%$), as illustrated in Fig. \ref{Throughput_500m_7Hz}. In particular, the top $20\%$ UEs have even achieved throughput gain of at least $1$ Mbits/s. As for UEs with poor channel condition (bottom $10\%$), C\&B shows great advantage over Max Power.

Finally, we present C\&B's advantages over all other candidate power control schemes based on the detailed performance summary in Table \ref{Table_PerformanceSummary}. C\&B shows desirable advantage over FPC by providing $51.9\%$ improvement on cell average throughput, while keeping the same $5\%$-Edge throughput performance and only dropping the power efficiency by $48\%$. Further, C\&B beats Max Power in significantly improving $5\%$-Edge throughput and power efficiency by $156\%$ and $5,716\%$ respectively, even with slightly increased cell average throughput. In comparison with the recently proposed CoMP scheme RLPC, C\&B achieves appreciable gains in cell average throughput and power efficiency respectively by $25.1\%$ and $71.2\%$, and simultaneous keeps $5\%$-Edge throughput slightly improved. 

Note that the performance improvement of C\&B is solely obtained by power control. One can further incorporate coordinated transceiver and scheduling techniques to achieve even higher gain. For example, it is known that CoMP receiving techniques can enhance the edge throughput significantly \cite{Suh11}. As shown in Table \ref{Table_PerformanceSummary}, the throughput gain of C\&B is more evident in the high throughput UEs. Hence, additional improvement is promising by combining C\&B with other CoMP techniques.

%On the contrary, as shown in Fig. \ref{IoT_500m_7Hz}, the time-average IoT has only increased by $1.5$ dB for almost all UEs. Compared to FPC scheme, C\&B boosts UEs' SNR  without significantly increasing UEs' experienced interference. As a consequence, the throughput performance is improved as shown in Fig. \ref{Throughput_500m_7Hz}. The throughput of good UEs (the top $40\%$) are noticeably improved. Especially the top $20\%$ UEs have achieved throughput gain of at least $1$ Mbits/s. The throughput of the rest UEs (the bottom $60\%$) are only slightly affected. As summarized in Table \ref{Table_PerformanceSummary}, the average throughput performance gain is $54.2\%$. with marginal loss in terms of $5^{th}$ percentile of UEs' average throughput, i.e. $5\%$-Edge throughput. This metic is widely used in industry to evaluate the performance of fairness among UEs. Though the power efficiency is only half of FPC, C\&B is still favorable due to the following reasons: (1) The key shortcoming of FPC is poor cell average throughput performance, in which C\&B is capable of providing significant improvement with marginal impact on fairness among UEs; (2) FPC has the best power efficiency among all existing power control schemes, which makes the the insignificant loss an acceptable compromise.
\begin{table}[h!]
\centering
\caption{Performance summary of FPC, Max Power, RLPC and C\&B in Macrocell Scenario.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|| c || c |  c | c | c ||}
 \hline
         & FPC & Max Power & RLPC & C\&B\\ 
 \hline
Average Throughput (Mbits/s) & $8.05$ & $12.01$ & $9.78$ & $12.23$     \\
\hline
$5\%$-Edge Throughput (Mbits/s)& $0.23$  & $0.09$ & $0.22$ & $0.23$   \\                                          
\hline
Power Efficiency (Mbits/J) & $751$ & $6.77$ & $226$ & $387$   \\                                       
\hline
\end{tabular}
}
\label{Table_PerformanceSummary}
\end{table}

%We also compare C\&B scheme with an alternative industrial power control scheme `Max Power', in which all UEs are transmitting at $P_{max}$. The cdf of UEs' average throughput is shown in Fig. \ref{Throughput_500m_7Hz}. It can be seen that the throughput performance of bottom $30\%$ and top $25\%$ UEs has been noticeably improved. The summary of results is shown in Table \ref{Table_PerformanceSummary}. We notice that the average throughput per sector and $5\%$-Edge throughput of Max Power scheme are $12.01$ and $0.09$ Mbits/s. Hence, C\&B scheme has achieved average and edge throughput performance gain of $3.33\%$ and $133\%$, respectively. Though the improvement on average throughput is little, C\&B has huge gain in edge throughput, which represents great performance in terms of fairness among different UEs. In other words, we are not sacrificing the poor UEs to boost the performance of good UEs. Furthermore, the power efficiency of C\&B is more than $53$ times better than that of Max Power. As illustrated in Fig. \ref{PowerEfficiency_500m_7Hz}, the power efficiency of every UE is improved by $10$ to $100$ times. Hence, compared with Max Power scheme, C\&B scheme can offer better throughput performance with $53$ times longer battery life. 
%To put this improvement into perspective, note that an iPhone $5$ battery has capacity, identical to $1.4$ Ahr. At $3.7$ V, this corresponds to approximately $20$K joules. On the other hand, at max power transmission, 200 mW is consumed during active transmissions. Given the fact that cellular transmissions correspond to $5-10\%$ of the overall consumption, a long file upload would drain a full battery to half in approximately 40mins under maximum power strategy. Our scheme increases this duration by a factor of \textbf{53}, which implies that, under our scheme, energy consumption for uplink transmission will no longer be a considerable fraction of energy consumption. Thus, even under continuous file uploads, the battery will run for more than a full day (assuming everything else is in normal operation mode).

%\begin{figure}
% \centering \includegraphics[width=2.5in]{PowerEfficiency_500m_7Hz.eps} \caption{Power Efficiency Performance.}
%\label{PowerEfficiency_500m_7Hz} \vspace{-0.cm}
%\end{figure}

%Note that the above calculations ignore the fact that, with maximum power pumped, the power amplifier and the transmission antenna will not operate in their most efficient region. Thus, there will be further losses with max power, due to lowered efficiency of the transmission circuitry.

%\begin{table}[h!]
%\centering
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{|| c || c |  c | c ||}
% \hline
%(Mbits/s)  & Max Power & C\&B & Improvement\\ 
% \hline
%Average Throughput  & $12.01$ & $12.41$   & \textbf{$3.33\%$}   \\
%\hline
%$5\%$-Edge Throughput & $0.22$  & $0.09$  & \textbf{144\%} \\ 
%\hline
%Power Efficiency (Mbits/J) & $6.77$ & $359$ &  \textbf{5,303\%} \\                                       
%\hline
%\end{tabular}
%}
%\caption{Throughput performance comparison between Max Power and C\&B.}
%\label{Table_CBvsMax}
%\end{table}

\subsubsection{Tradeoff between cell average throughput and cell edge throughput}

Recall the utility maximization problem (\ref{U_Maximize}), we can vary the weight parameter $\zeta$ to adjust the balance between received signal enhancement and interference mitigation. As we gradually decrease $\zeta$ from $1.3$ to $0.7$, the cell average throughput keeps improving in pair with the continuously degrading $5\%$-Edge throughput, as summarized in Table \ref{Table_DifferentWeight}. This tradeoff between average and edge throughput can be explained as follows: (a) the UEs with good channel conditions contribute most part of the average throughput. Increasing such UEs' transmission power by decreasing $\zeta$ greatly helps them to achieve stronger received signal, which results in their throughput gains. Such gains lead the cell average throughput to improve. (b) In contrast, boosting transmission power incurs stronger inter-cell interference, which especially jeopardizes those vulnerable UEs with poor channel states. As a result, the $5\%$-Edge throughput is decreased. 

\begin{table}[h!]
\centering
\caption{Throughput performance comparison between different weight factor $\zeta$ selections.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|| c || c |  c | c | c ||}
 \hline
       & $\zeta = 1.3$ & $\zeta = 1.1$ & $\zeta = 0.9$ & $\zeta = 0.7$\\ 
 \hline
Average Throughput (Mbits/s) & $12.23$ & $12.41$ & $12.95$   & $13.17$   \\
\hline
$5\%$-Edge Throughput (Mbits/s) & $0.23$ & $0.21$ &   $0.18$  & $0.15$ \\ 
\hline
\end{tabular}
}
\label{Table_DifferentWeight}
\end{table}

Note that when $\zeta = 0.7$, C\&B is remarkably better than the Max Power policy in terms of both average and edge-throughput. In addition, when $\zeta = 1.3$, C\&B is significantly better than the FPC and RLPC in term of cell average throughput. Therefore, one can adjust the weight parameter in order to adapt different system requirements.



%\subsubsection{Verification of Universality in Microcell Scenario}
%In order to verify the universality of C\&B, we execute the simulations in a microcell scenario where the inter-BS distance is reduced to $200$m. We set the weight parameter at $\zeta = 0.7$, in order to seek more improvement in cell average throughput. Switching $\zeta$ back to $1.3$ gives us similar performance as that in macrocell scenario.
%
%%The circumstance in microcell differs a lot from macrocell scenario: the shrunk cell size and increased user density makes UEs closer to their neighboring cells, which incurs significantly increased inter-cell interference. Such stronger interference greatly impairs UEs' SINR, which causes cell average throughput decrease. In particular, Max Power scheme fails to provide satisfactory improvement over FPC on cell average throughput due to the increasingly overwhelming interference incurred by overly high transmission power, but puts UEs with severely poor channel conditions (bottom $2\%$) in danger for getting nearly zero throughput. Thereby high cell average throughput is more preferable in microcell environment.   
%\begin{table}[h!]
%\centering
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{|| c || c |  c | c | c ||}
% \hline
%  & FPC & Max Power & RLPC & C\&B\\ 
% \hline
%Average Throughput (Mbits/s) & $6.60$ & $8.01$ & $6.61$ & $9.01$     \\
%\hline
%$5\%$-Edge Throughput (Mbits/s) & $0.20$  & $0.07$ & $0.34$ & $0.13$   \\                                          
%\hline
%Power Efficiency (Mbits/J) & $2838$ & $4.28$ & $970$ & $1338$   \\                                       
%\hline
%\end{tabular}
%}
%\caption{Performance summary of FPC, Max Power, RLPC and C\&B in Microcell scenario.}
%\label{Table_PerformanceSummary_200m}
%\end{table}
%
%C\&B continues to provide favorable improvements over all candidate power control schemes, as summarized in Table \ref{Table_PerformanceSummary_200m}. C\&B obtains cell average throughput gain by $36.3\%$ over both FPC and RLPC. Compared to Max Power, C\&B shows clear advantages from all three aspects: $12.5\%$, $85.7\%$ and $31,162\%$ improvements on cell average throughput, cell edge throughput and power efficiency, respectively. In addition, C\&B remains to offer $37.9\%$ higher power efficiency than RLPC. Therefore, C\&B is shown to supply performance improvements, universally to different cellular network scenarios.


%\begin{figure}
% \centering \includegraphics[width=2in]{figs/Throughput_200m_7Hz.eps} \caption{Time-average throughput in Microcell scenario.}
%\label{Throughput_200m_7Hz} \vspace{-0.cm}
%\end{figure}


==> GlobeCom16_Sumbmission/SystemModel.tex <==
\section{System Model and Problem Description}\label{SystemModel}
%In this paper, we consider uplink communication in LTE multicellular communication networks, where the cells (i.e. sectors) are divided into clusters (see Fig. \ref{Network_Model}). The remote BSs in each cluster are connected to a central BS, called eNodeB, which jointly manages the UEs in that cluster. Each UE is equipped with a single-carrier frequency division multiple access (SC-FDMA) air interface and the physical resource blocks (PRBs) are allocated in a contiguous fashion. Transmission block includes a Turbo encoder and a modulation and coding scheme that chooses the rates based on the 3GPP LTE standards. The receivers at BSs employ minimum mean square error (MMSE) detection, taking into account the available statistics of channel error, noise and interference. Also, interference rejection combination (IRC) techniques are implemented.
%\begin{figure}
% \centering \includegraphics[width=2.5in]{system.eps} \caption{Network Model.}
%\label{Network_Model} \vspace{-0.cm}
%\end{figure}
%
%The cellular system works in a discrete time pattern, with time slotted into transmission time intervals (TTI). TTI (1 ms as in LTE standards) refers to the duration of a transmission on the radio link, which is related to encapsulation of data from higher layers into frames. In each TTI, the receivers make estimations of UEs' instantaneous channel states based on the received pilot signals\footnote{The pilots include two types reference signals: Demodulation Reference Signal (DMRS) and Sounding Reference Signal (SRS). SRS is periodically transmitted for every UE to keep its CSI up to date at the BS. DMRS is transmitted along with one UE's data transmission}. With the accumulated channel state estimations, SINR predictions are calculated are forwarded to the adaptive modulation and coding (AMC) module. AMC selects the proper modulation and coding schemes (MCS) from given available adopted options, for each UE to maximize the throughput while satisfying the required block error rate (BLER) constraint. Afterwards, the scheduler select the UEs that are scheduled to transmit data, based on the feeding AMC decisions and consideration of fairness among different UEs. Finally, the scheduling and associated AMC decisions are transmitted to scheduled UEs by control signaling. Note that there exist propagation and processing delays related such control signaling, usually to be 6--8 TTIs. Power control has strong impacts on the strength of received pilot/data signals and the dynamics of experienced co-channel interference, and thereby crucially influence the performance of receiver estimation, AMC and scheduling.
%\subsection{Workflow of Real-life LTE Uplink Network}

%Consider a real-life LTE uplink networks, whose workflow is presented in Fig. \ref{WorkFlow}. One UE transmits data and pilots to its serving cell, while experiencing noise and interference from other UEs in neighboring cells. There exist two types of pilots: Demodulation Reference Signal (DMRS) and Sounding Reference Signal (SRS) \cite{36.213}. DMRS is only transmitted along with data and SRS is periodically transmitted from each UE. Both DMRS and SRS are used to estimate the instant channel gain. The results of channel estimation are then forwarded to the equalizer and decoder for detecting and decoding the transmitted data. In this process, the instant SINR is estimated and forwarded to the scheduler, together with the acknowledgement which indicates the success or failure of decoding. 

% and forwarded to the SINR predictor, together with the acknowledgement  which indicates success or failure of decoding. The predictor makes SINR predictions based on the accumulated SINR estimates and acknowledgements of decoding. The scheduler dynamically allocates PRBs to UEs according to their SINR predictions. Hence, the selection of active UEs and their allocated PRBs are changing from time to time. 
%\begin{figure}
% \centering \includegraphics[width=2.5in]{WorkFlow.eps} \caption{Workflow for pratical LTE uplink networks.}
%\label{WorkFlow} \vspace{-0.cm}
%\end{figure}

%The system is time slotted into transmission time intervals (TTI\footnote{TTI (set as in $1$ ms inLTE standards \cite{36.213}) refers to the duration of a transmission on the radio link, which is related to encapsulation of data from higher layers into frames.}). Note that there exists delay\footnote{Usually 6 to 8 TTIs in LTE networks.} of propagating and precessing the control signaling (e.g. outputs of power control and AMC) from the serving cells to UEs, thereby in each TTI, the scheduler makes SINR predictions according to the accumulated instant SINR estimates and acknowledgements of decoding. Based on the SINR predictions, scheduler selects the active UEs and allocates physical resource blocks (PRBs) to them for the upcoming TTIs. Here PRB refers to the unit of resource, which is set as the possession of $180$ kHz in frequency bandwidth and $1$ TTI in time \cite{36.213}. Hence, the active UEs and associated PRB assignments are dynamically decided by the scheduler from one TTI to another. The SINR predictions and scheduling decisions are then forwarded to the adaptive modulation and coding (AMC) module.
%The LTE system is time slotted into transmission time intervals (TTI\footnote{TTI (set as in $1$ ms in LTE standards \cite{36.213}) refers to the duration of a transmission on the radio link, which is related to encapsulation of data from higher layers into frames.}). In each TTI, the scheduler in each cell selects the active UEs and allocates the orthogonal subcarriers\footnote{One subcarrier has a bandwidth of $15$ kHz \cite{36.213}.} to them for the upcoming TTIs. Hence, the active UEs and associated subcarrier assignments are dynamically decided by the scheduler from one TTI to another, which causes dynamic inter-cell interference variations. 


%Every 12 subcarriers are grouped into one resource block (RB), with an inter-subcarrier spacing of $15$ kHz. Each RB  has a time slot duration of 1 millisecond, which consists of 12 or 14 OFDM symbols.\footnote{The actual number of OFDM symbols depends on the length of cyclic prefix.} In each cell, one UE use is scheduled to transmit on each RB, assigned with a transmission power and one modulation and coding scheme (MCS).

%The transmission power of each UE is determined by a power controller at its serving cell. 
%Besides open-loop power control, LTE standards, there are two types of power control: Open-loop and closed-loop. Open-loop power control is executed once every 50 time slots, which determines the transmission power based on large scale channel gain and interference level [??]. 
%In open-loop power control, each UE measures the strength of downlink reference signal (DRS) broadcast from neighboring cells, and selects the cell with the highest signal power as its serving cell \cite{36.213}, as illustrated in Fig. \ref{OLPC}. By channel reciprocity, the UE can estimates the large-scale path losses of its uplink wireless channels to nearby cells, which can be used to determine its uplink transmission power. 
%On top of open-loop power control, LTE standards also adopt closed-loop power control to adjust the transmission power in each time slots, based on instantaneous channel quality information \cite{36.213}.  
%\begin{figure}
% \centering \includegraphics[width=2in]{figs/OLPC.eps} \caption{Construction of open-loop power control.}
%\label{OLPC} \vspace{-0.cm}
%\end{figure} 

We consider an LTE uplink multicellular network. In such network, each UE transmits to its serving cell and meanwhile generates interference to its neighboring cells. Consider UE $u$ transmits signal $x$ at power $P$ on a single subcarrier, its received signal $y$ at the serving cell $c$ can be expressed as:
\begin{eqnarray}
y = \sqrt{P} \cdot h x + \sum_{j} \sqrt{P_j} \cdot h_{j}x_j + n, \label{Eq_ReceivedSignal}
\end{eqnarray}
where $h$ and $h_{j}$ denotes the instantaneous complex channel gain from UE $u$ and $u_j$ (served in neighboring cell $c_j$) to cell $c$, respectively, $n$ denotes the experienced noise. Hence the total inter-cell interference experienced by UE $u$ is $ \sum_{j} \sqrt{P_j} \cdot h_{j}x_j$. Assuming the transmitted signals $x$ and $x_j$ have unit variance, the signal-to-interference-plus-noise ratio (SINR) can thereby be calculated as:
\begin{eqnarray}
sinr =  \frac{P \cdot |h|^2}{ \sum_{j} P_j \cdot |h_{j}|^2 + \sigma_n^2}, \label{Eq_SINR}
\end{eqnarray}
where $\sigma_n^2$ denotes the variance of noise.

The power controller decides the transmission power of UEs across all cells, which heavily affects their SINR. Unlike Non-coordinated power control that only exploits the CSI of UEs to their serving cells, coordinated power control additionally utilizes the CSI of UEs to multiple neighboring cells. The problem we are tackling is to come up with a coordinated power control design with low complexity and high throughput gain over all existing solutions.
%The large-scale path loss between UE $u_j$ and cell $c_k$ is defined as: 
%\begin{eqnarray}
%PL_{jk} \triangleq \mathbb{E}\big[|h_{jk}|^2\big]^{-1},  \label{PL}
%\end{eqnarray} 
%where $\mathbb{E}[\cdot]$ denotes the expectation. When we only consider such large-scale path losses, $u_k$'s received signal-to-noise ratio (SNR) and interference over thermal noise (IoT) at $c_k$, and generated interference-to-noise ratio (INR) to $c_j$ can be respectively expressed as:
%\begin{eqnarray}
%SNR(P_k) &=& \frac{PL_{kk}^{-1} \cdot P_k}{N_0}, \label{Eq_SNR} \\
%IoT_k &=& \frac{N_0 + \sum_{j \neq k}{P_j \cdot PL_{jk}^{-1}}}{N_0}, \label{Eq_IoT}\\
%INR_{kj}(P_k) &=& \frac{PL_{kj}^{-1} \cdot P_k}{N_0}, \label{Eq_INR} 
%\end{eqnarray}
%where $N_0$ denotes the average noise power and is assumed to be the same and known for all UEs. Derived from Eq. (\ref{Eq_SNR}) and (\ref{Eq_IoT}), we can express the received signal-to-interference-plus-noise ratio (SINR) of UE $u_k$ as:
%\begin{eqnarray}
%SINR_k = \frac{SNR(P_k)}{IoT_k}. \label{Eq_SINR}
%\end{eqnarray}

Besides the strong impact from power controller, the throughput performance is also influenced by how each cell picks the modulation and coding scheme (MCS) for active UEs. In LTE networks, the existing Turbo-coded modulation techniques are paired with associated bit rate selections to form $29$ different available MCS options \cite{36.213}. For each SINR value, one of these MCS options is chosen by an Adaptive Modulation and Coding (AMC) module. The selected MCS should provide a sufficient high throughput and meanwhile guarantee a low decoding error probability. Usually, the block decoding error rate is required to be less than $10\%$, which will be later compensated by hybrid automatic repeat request (HARQ). The achievable throughput of one receiver design and the channel capacity  are illustrated in Fig. \ref{SINR-Throughput Mapping}. The stairs in the throughput curve are due to the AMC module. In particular, when the SINR is lower than $-6.5$ dB, no MCS can decode successfully and hence the throughput is zero. When the SINR is higher than $18$ dB, the maximum MCS can decode perfectly, achieving a maximum throughput. These features are common for any receiver design. 


%Assuming the same SINR is given, choosing high (low) transmission rate MCS results in high (low) block error rate (BLER). Therefore, the chosen MCS should be the one that maximizes the expected spectrum efficiency subject to the required target BLER constraint. Note that such maximized spectrum efficiency is only a function of SINR. We define this function as the SINR-Throughput mapping, i.e. $T(SINR)$.

%For each MCS $\gamma$, the assigned spectrum efficiency is $R(\gamma)$. Assuming SINR is given, the block error rate (BLER) is decided for each MCS by $\epsilon(\gamma, SINR)$\footnote{The function $\epsilon(\gamma,SINR)$ is related to the implemented physical layer techniques, including channel estimation, receiver beamforming, diversity, interference cancellation,etc.}. Thus, the AMC module selects the proper MCS $\gamma^*$ for each UE according to the given (imperfect) SINR information to maximize the achievable spectrum efficiency and subject to a given target BLER constraint $BLER_{target}$, i.e.maximized achievable spectrum efficiency with the selection of MCS $\gamma^*$, is only a function of SINR. We define this function as the SINR-Throughput mapping of AMC The SINR-Throughput mapping with perfect SINR information represents the best achievable spectrum efficiency, i.e. no further improvements can be made unless better MCS techniques are developed and adopted. 
%\begin{eqnarray}
%\gamma^* = & \arg \max_{\gamma \in \Gamma} &R(\gamma) \cdot \big[1-\epsilon(\gamma,SINR)\big] \label{PickMCS},\\
%\nonumber & s.t. &\epsilon(\gamma,SINR) \leq BLER_{target}
%\end{eqnarray}
%where $\Gamma$ denotes the set of all $29$ available MCS choices. It is important to see that the maximized achievable spectrum efficiency with the selection of MCS $\gamma^*$, is only a function of SINR. We define this function as the SINR-Throughput mapping of AMC, i.e. $T(SINR)$:
%\begin{eqnarray}
%T(SINR) \triangleq R(\gamma^*) \cdot \big[1-\epsilon(\gamma^*,SINR)\big] \label{Eq_T}
%\end{eqnarray}
%The SINR-Throughput mapping with perfect SINR information represents the best achievable spectrum efficiency, i.e. no further improvements can be made unless better MCS techniques are developed and adopted. 
 \begin{figure}
 \centering \includegraphics[width=2in]{figs/AMC_SINR-Throughput.eps} \caption{Throughput curve vs. channel capacity.}
\label{SINR-Throughput Mapping} \vspace{-0.2cm}
\end{figure}

%Fig. \ref{SINR-Throughput Mapping} illustrates the SINR-Throughput mapping generated according to our system-level simulation platform with perfect SINR information and $BLER_{target}$ set at $10\%$. We define the maximum value of $T(SINR)$ as $T_{\max}$, i.e.
%\begin{eqnarray}
%T_{\max} \triangleq \max_{SINR >0} T(SINR) \label{T_max}
%\end{eqnarray}
%Notice that $T(SINR)$ is a non-decreasing, finite and stair-shaped function, which performs considerably below the theoretical capacity due to block sizes and limited options of MCS. 

%In practice, the realistic spectrum efficiency is even worse due to the imperfect knowledge of SINR. Desirable power control solutions can help UEs to increase received SINR and achieve better knowledge of SINR information such that the realized spectrum efficiency is improved, which results in throughput performance gain. 


%Hence, power control plays a critical role in uplink cellular networks.


%Each cell decides the transmission power for its served UEs by power control. As shown in Fig. \ref{WorkFlow}, enhancing the signal strength of data/pilots and mitigating the inter-cell interference, which leads to increase the power of one UE and decrease the power of UEs in its neighboring cells, can both directly improve the performance of channel estimator, equalizer and decoder. Consequently, these improvements stimulate the scheduler and AMC module to perform better. Hence, power control plays a critical role in uplink cellular networks.

%Power control is operated by each cell, which decides the transmission power for its served UEs. Two types of power control are adopted in LTE uplink networks: open-loop and closed-loop. Open-loop power control sets the basic operational transmission power for each UE in a slow mode, i.e. the system only executes open-loop power control once in every tens (e.g. 50) of TTIs. Closed-loop power control makes adaptive adjustments on top of open-loop power allocation in each TTI that one UE is active. This adjustment is made based on the feedback from the receiver at each cell. The general construction of all existing open-loop power control schemes is presented in Fig. \ref{OLPC}, where cells broadcast downlink reference signals (DRS) to UEs. Each UE selects the cell with the highest reference signal received power (RSRP) \cite{36.133} as the serving cell. Each UE also estimates the large-scale path losses based on RSRP for all nearby cells \cite{Rao07} and forward to its serving cell. These estimates are regarded as the uplink large-scale path losses due to the channel reciprocity. Based on the path loss information, open-loop power control decides the transmission power and send control signaling to the corresponding UE. 
%It is worth emphasizing that the SINR-throughput mapping $T(SINR)$ is a system priori and can be easily achieved by the power controller with only a one-time forward from the AMC module. However, it has not been used by any existing open-loop power control approach.

%\subsection{Large-scale System}
 %Open-loop power control allocates transmission power Fig. \ref{System_Model} represents an illustrative example of LTE uplink network. Three UEs that served in different cells are assigned with the same physical-layer resource block (PRB). $G_{ij}$ denotes the large-scale channel gain from UE $u_i$ to cell $c_j$ ($i,j \in \{1,2,3\}$). Its inverse, i.e. $G_{ij}^{-1}$, is defined as the large-scale path loss $PL_{ij}$. Consider UE $u_i$ to be allocated with transmission power $P_i$ by open-loop power control,
 
%$u_k$'s received large-scale Signal-to-Noise Ratio (SNR), Signal-to-Interference-plus-Noise Ratio (SINR), Interference-over-Thermal (IoT) at its serving cell $c_k$, and generated large-scale Interference-to-Noise Ratio (INR) to its neighboring cell $c_j$ can be calculated as below:
%\begin{eqnarray}
%SNR(P_k) &=& \frac{PL_{kk}^{-1} \cdot P_k}{N_0}, \label{Eq_SNR} \\
%SINR_k &=& \frac{PL_{kk}^{-1} \cdot P_k}{N_0 + \sum_{j \neq k}{P_j \cdot PL_{jk}^{-1}}}, \label{Eq_SINR} \\
%IoT_k &=& \frac{N_0 + \sum_{j \neq k}{P_j \cdot PL_{jk}^{-1}}}{N_0}, \label{Eq_IoT} \\
%INR_{kj}(P_k) &=& \frac{PL_{kj}^{-1} \cdot P_k}{N_0}, \label{Eq_INR} 
%\end{eqnarray}
%where $N_0$ denotes the average noise power and is assumed to be the same for all UEs. $PL_{kj}$ denotes the large-scale path loss from UE $u_k$ to its neighboring cell $c_j$. The above large-scale metrics are widely used in existing open-loop power control schemes for parameter selection \cite{Coupechoux11}-\cite{Yang09}. We will exploit these metrics in our power control design from a different point of view.

%\begin{figure}
% \centering \includegraphics[width=2.5in]{System_Model.eps} \caption{An illustrative example of uplink cellular networks.}
%\label{System_Model} \vspace{-0.cm}
%\end{figure}


==> Principles.tex <==
\section{Challenges of Practical Power Control}\label{Principles}

%The objective of open-loop power control is to adjust UEs' transmission power, such that strong enough received signal is guaranteed and severe co-channel interference is avoided. Moreover, the construction of power control is subject to a number of constraints in real-life cellular systems, e.g. huge number of involved cells, complicated environment circumstances, numerous UEs with various mobility, etc. Therefore, it requires open-loop power control to have following properties:
The task of uplink power control is to determine the transmission power of each UE, such that the signal received  at the base station is sufficiently strong, and the interference generated to nearby base stations is not severe. In reality, this task is arduous because of many factors, such as enormous users and cells, complicated propagation environment, and dynamic user mobility. These factors impose the following requirements in the design of uplink power control:
\begin{itemize}
\item \textbf{Efficient:} High throughput is required to meet the requirement of cellular systems.
%High throughput is provided to satisfy the communication speed requirements of current (e.g. 3G, LTE) and next generation (e.g. 5G, 6G) cellular systems.

\item \textbf{Reliable:} The channel condition and interference power may vary acutely over time. For example, a strong interference source may exist in one slot and disappear in the next slot because of dynamic scheduling. The quality of service is required be sufficiently high in such scenarios.

\item \textbf{Fair:} The uplink throughput varies from one UE to another, which can be quite low for UEs with poor channel conditions. The power controller needs to reduce the interference level such that the  5-percentile throughput, which is usually termed cell-edge throughput, is sufficiently high.
%Guarantee acceptable performance for UEs that have poor channel and/or confront strong interference. The throughput of these UEs, measured by $5$ percentile throughput (i.e. $5\%$-Edge throughput), is greatly lower than the average and indicates the fairness among UEs.

\item \textbf{Autonomic:} UEs' power allocation within once cell is decided independently from UEs in other cells. No assistance from other UEs/cells, control signaling exchange/iterations with other power control modules, or feedback is needed.

%\item \textbf{Simple:} The computational and implementational complexity is low. UEs' connection establishment process is simplified, performance analysis and adaptive adjustment can easy to be made.

\item \textbf{Universal:} The power control algorithm must be universally applicable in all system circumstances, which differ in cell size, UE density, mobility speed, and path loss factor.
\end{itemize}

In practice, overly high and overly low transmission powers are both harmful. Specifically, increasing the transmission power of one UE can increase its  throughput, and meanwhile cause strong interference to nearby cells which will degrade the throughput of other UEs. Hence, there is a tradeoff between signal enhancement (SNR) and interference mitigation (INR). In real systems, it is extremely difficult, if not impossible, to find the optimal tradeoff point between SNR and INR because there are a huge population of users with diverse channel conditions, and channel knowledge is only available for a small amount of local wireless links. Existing power control algorithms \cite{Whitehead}-\cite{Rao07} usually determine the transmission power based on a simple heuristic linear equation with one or two parameters, and explore different tradeoff points by adjusting these parameters. So far, there is little success to improve these algorithms, because of the complicated tradeoff between SNR and INR and the practical requirements mentioned above. 
%All of the above requirements are crucial to a desirable open-loop power control solution. Universality and robustness together decide whether the proposed solution can be widely adopted. Efficiency and fairness guarantee the designed scheme to satisfy diverse quality of service (QoS) requirements. UE-Independence and Simplicity lead a open-loop power control scheme to be implemented in practical systems due to the low investment cost and infrastructure requirement. 
In the following section, we propose our open-loop power control scheme that has all these valuable properties. 

